Computing conjugate barrier information for nonsymmetric cones

The recent interior point algorithm by Dahl and Andersen [10] for nonsymmetric cones as well as earlier works [16,19] require derivative information from the conjugate of the barrier function of the cones in the problem. Besides a few special cases, there is no indication of when this information is efficient to evaluate. We show how to compute the gradient of the conjugate barrier function for seven useful nonsymmetric cones. In some cases this is helpful for deriving closed-form expressions for the inverse Hessian operator for the primal barrier.

==> numerical.tex <==
\section{Numerical Verification}
\label{sec:numerical}

Conjugate gradients can always be evaluated by solving \cref{eq:gpdef} using Newton's method, which we refer to as the \emph{generic approach}.
In this section our aim is to verify empirically that the Newton-Raphson method for calculating the $\tg$ oracle of $\khpower$, $\krpower$, and $\kinf$ converges in a very small number of iterations from our chosen initial points.
We also demonstrate that the generic approach can require tens or hundreds of iterations at the same points (as mentioned in \cref{sec:introduction}, this renders the approach useless for interior point solvers).
% In this section we compare the numerical properties and computational efficacy of the conjugate gradient procedures from \crefrange{sec:sumlog}{sec:inf} against the generic approach.
We test both approaches by evaluating conjugate gradients at randomly generated points in the dual cone.
Since the procedures for $\klogdet$, $\krtdet$, and $\kspec$ mirror those of $\klog$, $\khgeom$, and $\kinf$, we omit the matrix variants for brevity.

We implement the generic approach as follows.
The objective in \cref{eq:gpdef} is self-concordant.
As described by \cite[Section 5.2]{nesterov2018lectures}, the objective can be optimized by combining the damped Newton's method with the full Newton's method.
In particular, the Hessian $H$ of $f$ induces a local norm at any $w \in \K$ that is given by $\lVert z \rVert_w = \sqrt{\langle z, H(w)^{-1} z \rangle}$ for all $z$.
When the local norm of the gradient of the objective, that is $\lVert r + g(w) \rVert_w$ is less than $\tfrac{3 - \sqrt{5}}{2}$, Newton's method begins to converge quadratically.
We stop iterating when the local norm of the gradient is lower than some tolerance $\epsilon$.
In our experiments we set $\epsilon$ to $1000$ times machine precision.
Alternatively, we stop if we detect insufficient progress between consecutive iterations (stalling).
The procedure is summarized in \cref{proc:conjgrad}.
%
\begin{algorithm}[!htb]
\caption{Newton's method for computing a conjugate gradient.}\label{proc:conjgrad}
\begin{algorithmic}[1]
\Procedure {compute $g^\ast(r)$}{} \\
\algorithmicrequire { $r$, $\epsilon$, $w_0$, oracles for $g(w)$, $H(w)^{-1}$}
\State $w \gets w_0$
% \State $z \gets g(w) + r$
\State $\lambda_1 \gets \sqrt{\langle g(w) + r, H(w)^{-1} (g(w) + r) \rangle} = \sqrt{\nu - 2 \langle w, r \rangle + \langle r, H(w)^{-1} r \rangle}$
\State $j \gets 1$
\While {$\lambda_j > \epsilon$}
\If {$\lambda_j > \tfrac{3 - \sqrt{5}}{2}$}
\State $\alpha \gets (1 + \lambda_j)^{-1}$
\Comment {damped Newton's method}
\Else
\State $\alpha \gets 1$
\Comment {full Newton's method}
\EndIf
\State $w \gets w - \alpha H(w)^{-1} (g(w) + r)$
% \State $z \gets g(w) + r$
\State $\lambda_j \gets \sqrt{\langle g(w) + r, H(w)^{-1} (g(w) + r) \rangle} = \sqrt{\nu - 2 \langle w, r \rangle + \langle r, H(w)^{-1} r \rangle}$
\If {$\lambda_j > \tfrac{3 - \sqrt{5}}{2}$ and $\lambda_j > 1000 \big( \tfrac{\lambda_{j-1}}{1 - \lambda_{j-1}} \big)^2$}
\State \textbf{break} 
\Comment{slow progress}
\EndIf
\State $j \gets j + 1$
\EndWhile
\State \Return $-w$
\EndProcedure
\end{algorithmic}
\end{algorithm}

For each of the cones $\klog$, $\khgeom$, $\khpower$, $\krgeom$, $\krpower$, we generate a random dual point by generating a random $r_i$ variable in $(0, 1)$ for $i \in \iin{d}$ and for $\klog$, we also generate a random perspective variable $p$.
We generate the epigraph/hypograph variable ($p$ or $q$) by letting the relative violation on the epigraph/hypograph inequality in the cone equal some offset fraction $o \in (0, 1)$.
For example, for $\klog$, given randomly generated $r$ and $p$, we let:
\begin{subequations}
\begin{align*}
    \bar{q} &= p \tsum_{i \in \iin{d}} \log (-\tfrac{r_i}{p}) + p d,
    \\
    q &= \bar{q} \times (1 + \sgn(\bar{q}) \times o),
\end{align*}
\end{subequations}
which ensures $(p, q, r) \in \intr(\klog^\ast)$ and $o$ controls proximity to the boundary.
Points that are very near to the dual cone boundary are generally visited near the end of an interior point algorithm, and it is particularly important for the $\tg$ oracle to return accurate values at those points.
% At each dual point $r$, we measure violation on \cref{eq:grdot}:
% \begin{align}
%     \lvert \langle g^\ast(r), r \rangle + \nu \rvert,
%     \label{eq:residual}
% \end{align}
% where $\tg(r)$ is obtained by one of two procedures.
% Note that the term inside the absolute value of \cref{eq:residual} should be positive as long as the estimated $-\tg$ is in $\K$, but could be negative from numerical error.
At each dual point $\tp$, we check the violation on \cref{eq:grdot}:
\begin{align}
    \lvert \langle g^\ast(\tp), \tp \rangle + \nu \rvert.
    \label{eq:residual}
\end{align}
The residuals on \cref{eq:residual} from the two procedures are comparable (often within a factor of $100$ of each other or more favorable for the specialized methods) so we do not report on the accuracy differences.
We count the number of Newton iterations taken by the generic approach and if applicable, the number of steps taken by the Newton-Raphson methods from \cref{lem:hpower,lem:rpower,lem:inf}.
In \cref{tab:iters} we give the average number of iterations from each approach over 10 randomly generated points (and randomly generated $\alpha$ for $\khpower$ and $\krpower$).
% Recall that an iteration of the generic Newton's method requires applying an inverse Hessian matrix of side dimension $d$.
% It is clear that each iteration of the generic Newton's method is much more expensive then an iteration of a univariate Newton-Raphson method or evaluating the conjugate gradient in closed form.
In all experiments the generic approach requires tens or hundreds of iterations (which are mostly damped Newton iterations), and the number of iterations grows as $d$ increases and the offset from the boundary $o$ decreases.
For the specialized conjugate gradient procedures, the iteration counts remain fairly constant (usually $2$--$6$) for different $d$.
Experiment code can be found at \url{https://github.com/lkapelevich/conjgradexperiments}%
\footnote{%
In our implementation we calculate $h'$ and take the Newton-Raphson step in quad precision (using the \texttt{DoubleFloats.jl} \cite{julia2022double} package in  Julia), which is relatively inexpensive (since it only involves elementary operations on scalars and not any matrices or vectors) and only affects our results for $\kinf$.
}.


\begin{table}[!htb]
\sisetup{
table-text-alignment = right,
table-auto-round,
table-figures-integer = 4,
table-figures-decimal = 1,
table-format = 4.1,
add-decimal-zero = false,
% add-integer-zero = false,
}
    \begin{tabular}{ll*{11}{r}}
    \toprule
        $d$ & $o$ & $\klog$ & \multicolumn{2}{c}{$\khpower$} & $\khgeom$ & \multicolumn{2}{c}{$\krpower$} & $\krgeom$ & \multicolumn{2}{c}{$\kinf$} \\
        \cmidrule(lr){4-5} \cmidrule(lr){7-8} \cmidrule(lr){10-11} 
        & & g & g & s & g & g & s & g & g & s  \\
        \midrule
        \multirow{5}{*}{20} 
& $10^{-5}$ & 98. & 88. & 2.0 & 27. & 88. & 3.0 & 27. & 41. & 2.0\\ 
& $10^{-4}$ & 84. & 74. & 2.0 & 27. & 74. & 3.0 & 27. & 36. & 3.0\\ 
& $10^{-3}$ & 70. & 61. & 3.0 & 27. & 60. & 3.0 & 27. & 30. & 4.0\\ 
& $10^{-2}$ & 56. & 46. & 3.0 & 27. & 46. & 4.0 & 26. & 24. & 5.0\\ 
& $10^{-1}$ & 40. & 31. & 4.0 & 25. & 31. & 4.0 & 24. & 17. & 5.0\\ 
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{5}{*}{40} 
& $10^{-5}$ & 196. & 130. & 2.0 & 37. & 127. & 3.0 & 37. & 46. & 3.0\\ 
& $10^{-4}$ & 160. & 108. & 2.0 & 37. & 105. & 3.0 & 37. & 40. & 4.0\\ 
& $10^{-3}$ & 124. & 85. & 3.0 & 37. & 83. & 3.0 & 37. & 34. & 5.0\\ 
& $10^{-2}$ & 90. & 63. & 3.0 & 37. & 62. & 3.4 & 36. & 27. & 6.0\\ 
& $10^{-1}$ & 57. & 41. & 4.0 & 33. & 41. & 4.0 & 33. & 19. & 5.0\\ 
\addlinespace[2pt]
\hdashline
\addlinespace[2pt]
\multirow{5}{*}{60} 
& $10^{-5}$ & 301. & 218. & 2.0 & 46. & 211. & 3.0 & 45. & 49. & 3.1\\ 
& $10^{-4}$ & 240. & 170. & 2.0 & 46. & 164. & 3.0 & 45. & 44. & 4.3\\ 
& $10^{-3}$ & 180. & 124. & 3.0 & 46. & 120. & 3.0 & 45. & 38. & 5.5\\ 
& $10^{-2}$ & 124. & 83. & 3.0 & 45. & 81. & 3.0 & 44. & 30. & 6.0\\ 
& $10^{-1}$ & 76. & 50. & 4.0 & 40. & 49. & 4.0 & 39. & 21. & 5.0\\ 
        \bottomrule
    \end{tabular}
    \caption{Mean number of iterations using a generic Newton method (g), and when applicable, univariate Newton-Raphson from specialized methods (s) over 10 random points.}
    \label{tab:iters}
\end{table}


